Dialing back time on Timepix3: A study on the timing performance of Timepix3

For the advancement of the understanding of timing systematics in pixelized readout chips and for the benefit of future fast timing detectors to aid 4D tracking technology in the HL-LHC, we have performed detailed studies of the timing properties of the Timepix3, a hybrid pixel detector developed by the Medipix collaboration. These studies use three different measurement techniques to investigate the timing systematics of this detector: test pulses, testbeam, and a laser setup that we build for this work. The average delay over the pixel matrix is determined with the testbeam and the laser and shows the same structure for different Timepix3 chips. The difference in delay results in a maximum difference over the pixel matrix of around 4 ns, which is large compared to the time bins of 1.56 ns. By correcting for this difference on a per-pixel level, the time resolution is on average improved with 159 ps depending on the sensor. The best time resolution that is achieved after a timewalk correction and a correction for the difference in the average delay per pixel is 686.4$\pm$0.2 ps for a single Timepix3 chip with a 200 $\mu\text{m}$ planar silicon sensor, compared to a time resolution of 892.9$\pm$0.3 ps without any correction. However, this improved time resolution is not yet the naively expected time resolution of 451 ps. The origin of this delay is determined with this laser setup, and is due to a combination of signal propagation and a difference of the start-up time of the fast oscillator within the pixels. This work indicates that it is vital for next generation pixel detectors to correct for these systematic timing effects in order to reach a better time resolution to aid 4D tracking technology in the HL-LHC.

==> Chapters/Discussion.tex <==



\chapter{TODO:Discussion}
\label{sec:Discussion}



==> Chapters/Theory/LaserTheory.tex <==


\section{Principles of a Laser}

\subsection{Bandwidth of Laser}
\label{sec:Theory/LaserTheory}

A Light Amplification by Stimulated Emission of Radiation (laser) diode is able to produce a high-power coherent focused laser beam. Most lasers however, still exhibit a fairly broad bandwith. To limit the laser's bandwith to below \SI{1}{\nano\meter}, a Fibre Bragg Grating (FBG) can be used. A FBG consists of a periodic perturbation of the refractive index in the core of an optical fibre. This structure leads to the reflectance of a narrow frequency band, for which the Bragg condition is satisfied \citep{hill1997fiber}:
\begin{equation}
    \frac{2 \pi}{\Lambda} = 2 \frac{2 \pi n_{eff}}{\lambda}\ \ \rightarrow \ \ \lambda = 2n_{eff}\Lambda.
\end{equation}
$\Lambda$ is the grating period, $\lambda$ the wavelength of the light, and $n_{eff}$ is the effective refractive index. This effective refractive index is in many ways similar to the normal refractive index that will be discussed later on, however the effective refractive index is intimately tied to the idea of waveguides instead of free space. The effective refractive index gives the ratio of the velocity of light in vacuum to the velocity of a mode for a given polarization in the direction of propagation in a waveguide, and thus is only defined within a waveguide. 

When the Bragg condition is satisfied, the complex amplitudes corresponding to the reflected field from different parts of the grating are all in phase \citep{hill1997fiber}. This phase-matching is crucial for the total transmission of the narrow band, only when this phase-matching is achieved, the different components of the electric field from the different parts of the grating add up constructively and only the narrow band is transmitted. FBGs are commonly used in combination with a laser diode to make a single-frequency laser diode with a sub-nanometer bandwidth or are used as frequency filters in optical communication \citep{udd2011fiber}. A FBG can also be used as the end mirrors of the laser resonator instead of outside the laser to form a distributed feedback laser \citep{lizarraga2009single}. The laser that is used in this Thesis is a FBG wavelength stabilized single mode laser, which has a bandwidth of less than \SI{1}{\nano\meter}.

For a detailed explanation on the physics of lasers see \citep{Koechner2003}, and for a more detailed explanation on FBGs see \citep{hill1997fiber}.






\subsection{Propagation of Laser Beam in Free Space}
\label{sec:Theory/PropLaserBeam}
The light that is generated by a laser, can be manipulated in multiple ways. One of them is with the use of lenses, which can for example expand or collimate the laser beam. For the laser setup that is used later on, it is important to understand the shape of a laser beam after it is focused to a narrow point. Therefore, this phenomena will be discussed in this Section. 

After focusing a parallel beam of light using a single lens, in general the focusing of the light will not be in a perfect straight cone, but will form a parabolic shape. For lenses with a big diameter and large focus spots, this cone is well approximated by a normal straight cone, however when a relatively small spot size is desired, the shape of the beam around the focus point starts to depend on the wavelength, lens diameter, and spot size. To calculate the beam shape around the focus point, a Gaussian beam profile is assumed. The transverse profile of the optical density $I$ of a Gaussian beam with power $P$ can be described with the Gaussian function \citep{varga1998gaussian}:
\begin{equation}
    I(r,z)=\frac{2P}{\pi w^2\left(z\right)}\exp(-2\frac{r^2}{w^2\left( z \right)}),
\end{equation}
where $w\left( z \right)$ is the beam radius at $z$. The beam radius is defined as the radius at which the intensity has dropped to a factor $1/e^2$ of the maximum intensity. Gaussian beams are generally only considered when the beam divergence is small. Because of the small divergence, the Fresnel approximation \citep{Steane:89} (also known as the paraxial approximation) can be applied. This approximation assumes that normal vector of the wave front at any position within the beam is only slightly deviating from the beam axis were the angle between them is given by $\theta$. This condition then implies $\sin(\theta)\approx\theta,\tan(\theta)\approx\theta, \ \text{and}\ \cos(\theta)\approx1$. By applying this approximation, the second-order derivative in the propagation equation can be omitted. This propagation equation can be derived from Maxwell's equation, and becomes a first order differential equation after omitting the second-order derivative. For a Gaussian beam, the time and space dependence is given by \citep{varga1998gaussian}
\begin{equation}
    E(r,z;w_0)=E_0\frac{w_0}{w\left( z \right)}\exp[-r^2\left( \frac{1}{w^2\left( z \right)} -\frac{ik_0}{2 R\left( z \right)} \right)-i\Phi\left( z \right)],
    \label{eq:Theory/EField}
\end{equation}
where 
\begin{align}
  \phantom{w^2\left( z \right)}
  &\begin{aligned}
    \mathllap{w^2\left( z \right)} &= w_0^2\left( 1+\frac{z^2}{z_0^2} \right),
  \end{aligned}\\
  \phantom{w^2\left( z \right)}
  &\begin{aligned}
    \mathllap{R\left( z \right)} &= z\left( 1+\frac{z^2}{z_0^2} \right),
  \end{aligned}\\
  \phantom{w^2\left( z \right)}
    &\begin{aligned}
    \mathllap{\Phi\left( z \right)} &= \arctan(\frac{z}{z_0}),
  \end{aligned}\\
    &\begin{aligned}
    \mathllap{z_r} &= \frac{\pi w_0^2}{\lambda}.
    \label{eq:Theory/Laser/Rayleigh}
  \end{aligned}
\end{align}
Here, $k$ is the wavenumber of the light in the beam, and is given by $k=2\pi/\lambda$. $z_r$ is known as the Rayleigh length, and gives an indication over which length the beam can propagate without deviating significantly in radius. The beam waist $w_0$ can be expressed in terms of the wavelength and the angular width $\theta$ of the beam \citep{varga1998gaussian}:
\begin{equation}
	w_0=\frac{2 \lambda}{\pi \theta}.
    \label{eq:Theory/beamWaist}
\end{equation}

The real part of the electric field can be obtained by multiplying \autoref{eq:Theory/EField} with $\exp(-2i\pi c t / \lambda)$, where $c$ is the speed of light. The real part of the electric field for a wavelength of 680 \si{nm} with a beam waist radius of $\SI{7}{\micro\meter}$ is shown in \autoref{fig:Theory/EFieldSpot}. For a complete derivation of the solution for a Gaussian beam see \citep{varga1998gaussian}.


\begin{figure}
\centering
\begin{minipage}{.47\textwidth}
\centering
\includegraphics[width=1\linewidth]{Figures/Theory/EFieldSpot.png}
\end{minipage}\qquad
\begin{minipage}{.47\textwidth}
\centering
% the intensity profile of the beam should be placed here
\includegraphics[width=1\linewidth]{Figures/Theory/IFieldSpot.png}
\end{minipage}

%\bigskip

\begin{minipage}[t]{.47\textwidth}
\centering
\captionsetup{width=.9\linewidth}
\captionof{figure}{An example of the electric field for a Gaussian beam that is focused to a radius of \SI{7}{\micro\meter}. The Gaussian beam is travelling towards the negative height direction.}
\label{fig:Theory/EFieldSpot}
\end{minipage}\qquad
\begin{minipage}[t]{.47\textwidth}
\centering
\captionsetup{width=.9\linewidth}
\caption{The intensity profile of the electric field shown in \autoref{fig:Theory/EFieldSpot}.}
\label{fig:Theory/IFieldSpot}
\end{minipage}
\end{figure}

The intensity profile for the the propagating beam can also be calculated using \autoref{eq:Theory/EField}. The relation between the electric field and the intensity is given by \citep{hecht2016optics}
\begin{equation}
    I(z,r)=2nc\epsilon_0\abs{E(z,r)}^2.
\end{equation}

Here $n$ is the refractive index of the medium in which the beam is propagating. The intensity profile for the electric field shown in \autoref{fig:Theory/EFieldSpot} is shown in \autoref{fig:Theory/IFieldSpot}. It can be noted that with a beam waist of $\SI{7}{\micro\metre}$, the height variation for which the intensity stays within a value of $1/e^2$ of the maximum value is just $\SI{226}{\micro\metre}$. Therefore it becomes more difficult to find the focal point for profiles with a beam waist of less than $\SI{7}{\micro\metre}$. Precise control of the position of the lens used to focus the beam is thus often required for beam waists in this order of magnitude.

\subsection{Focusing of Laser Beam}
\label{sec:Theory/FocusLaser}
To be able to focus a laser beam to a few \si{\micro\meter} it is important to choose the correct lens or lenses. In the case of a Gaussian profile, two equations govern the spot size that can fundamentally be achieved. The first one is due to the imaging of the fibre to the position of the focal point. A lens system images an object before the lens, to an image after the lens. By choosing the focal length and position of the object and image, a specific magnification can be achieved. Depending on the application of the lens, this magnification can be greater or smaller than one. 

For the laser setup that is used later on (see \autoref{sec:LaserSetup}), the output of the fibre will be imaged to the focal point. Therefore, a fundamental limit by this imaging on the spot size can be determined. For a two lens system, in which the first one collimates the light ($f_{in}$), and the second one focuses it ($f_{out}$), the magnification is given by the ratio of the second lens over the first lens \citep{Goodman:85}. Therefore, the minimum spot size due to imaging is
\begin{equation}
	d_{spot}=\frac{f_{out}}{f_{in}}d_{fiber}.
\end{equation}

The second constraint on the size of the focal spot is due to the beam waist approaching, but never reaching zero. To determine this size, \autoref{eq:Theory/beamWaist} can be rewritten to find an expression for the angular width of the beam. This yields
\begin{equation}
	\theta = \frac{4\lambda}{2 \pi w_0}.
    \label{eq:Theory/angularWidth1}
\end{equation}
The angular width can also be geometrically be determined assuming that the beam covers the complete lens, which has a diameter of $D$. The angular width is given by
\begin{equation}
	\theta=2\tan{\left(\frac{D}{2f_{out}}\right)} \approx \frac{D}{f_{out}}.
    \label{eq:Theory/angularWidth2}
\end{equation}
The paraxial approximation is again used to approximate $\tan(x)$ as $x$. 

By equating \autoref{eq:Theory/angularWidth1} to \autoref{eq:Theory/angularWidth2}, an expression for the beam waist can be found as a function of the properties of the second lens. The beam waist is given by
\begin{equation}
	w_0 = \frac{4\lambda}{\pi}\frac{f_{out}}{D}.
\end{equation}

However, this beam waist can never be reached if the image size of the initial object is bigger than this beam waist. Therefore the diameter of the minimal spot size is given by
\begin{equation}
	d_{min,spot}=\text{min} \left\{\frac{f_{out}}{f_{in}}d_{fiber}, \ \frac{4\lambda}{\pi}\frac{f_{out}}{D} \right\}.
    \label{eq:Theory/minSpotsize}
\end{equation}



\subsection{Interactions with Matter}
\label{sec:Theory/InteractionWithMatter}
Another important aspect to understand is the interaction of light with matter. In this Section the reflection and absorption of light in matter as well as the generation of charge carriers by a high energy charged particles are discussed. 

When light encounters a change of medium, there are two possibilities that could happen: reflection, or transmission. The amount of reflection and transmission depends on a few variables such as the index of refraction of the two materials, and the frequency of the light. The refractive index of a material consists of two parts: a real and an imaginary part. To understand what effect each part has on the light, one can look at what it does to a fictitious electric field $E(x)$ described by $E(x)=\exp(i\frac{\omega x}{c})$. In a material with refractive index $n$, this electric field is described by $E(x)=\exp(i\frac{n\omega x}{c})$. This electric field will propagate at a different frequency and a slower speed, however, this does not yet describe the absorption of the electric field in the medium. The complex refractive index is needed to describe the absorption of the electric field within a medium. The complex refractive index can written as $n'=n+i\kappa$. The electric field in the medium can now be described by two exponents:
\begin{equation}
    E(x)=e^{-\frac{\kappa\omega}{c}}e^{i\frac{n\omega x}{c}}.
\end{equation}
The first term describes the absorption in the medium and the second term the wave propagation of the electric field in the medium. Without the imaginary part of the refractive index, it is impossible to describe the decay of the electric field within the medium. For a more detailed introduction to the (complex) refractive index see \citep{hecht2016optics}.

\begin{figure}
\centering
\includegraphics[width=.75\linewidth]{Figures/Theory/SiAbsDepth.png}
\captionof{figure}{The absorption depth of optical photons with various wavelengths in the (near-)optical range. The absorption coefficients to calculate the absorption depth are taken from \citep{green1995optical}.}
\label{fig:Theory/SiAbsDepth}
\end{figure}

The values of $n$, and $\kappa$ also depend on the wavelength of the photon. For example, x-rays are almost not absorbed in thin pieces of material, while \SI{600}{\nano\meter} photons are absorbed within \SI{15}{\micro\meter} of material. For silicon, the values of $n$ and $\kappa$ in the optical range are investigated by \citet{green1995optical}. Green \& Keevers also calculated the absorption coefficient of silicon. The absorption coefficient $\mu_{abs}$ is the length over which the original intensity has dropped to a factor $1/e$ of the original intensity. The absorption depth $\lambda_{abs}$ can be calculated with the absorption coefficient by $\lambda_{abs}=\mu_{abs}^{-1}$ \citep{hecht2016optics}. The absorption depth for silicon in the optical range is shown in \autoref{fig:Theory/SiAbsDepth}. The bandgap energy of silicon is \SI{1.12}{\eV}, which is the same energy as a photon with a wavelength of \SI{1107}{\nano\meter}. Photons with a wavelength of more than \SI{1107}{\nano\meter} are therefore less likely to be absorbed by the silicon. This explains the rapidly increasing absorption depth at higher wavelengths.

Besides the influence of the wavelength on the absorption depth, the reflection and transmission on the silicon interface also depends on the wavelength of the photons as well as on the angle of incidence. These relations are known as the Fresnel equations and are for p-polarized light given by \citep{hecht2016optics}
\begin{align}
    r_p&= \frac{n_1\cos(\theta_t) - n_2\cos(\theta_i)}{n_1\cos(\theta_t)+n_2\cos(\theta_i)}, \\ 
    t_p&= \frac{2n_1\cos(\theta_i)}{n1\cos(\theta_t)+n_2\cos(\theta_i)},
\end{align}
where the relation between the angle of incidence $\theta_i$ and the angle of the reflected light $\theta_t$ is given by Snell's law \citep{hecht2016optics}.
The intensity of the reflection however, is not simply given by $r_p$. The fraction of the intensity that is reflected at the interface is given by \citep{hecht2016optics}
\begin{equation}
    R=\frac{\abs{E_r}^2}{\abs{E_i}^2}=\abs{r}^2.
\end{equation}
The fraction of the intensity that is transmitted at the interface is now given by the fraction that is not reflected: $T=1-R$. The complete derivation of these equations as well as the expressions for s-polarized light can be found in \citep{hecht2016optics}. 

Using these expressions for the reflectance, the reflectivity of silicon can be calculated. In the case of silicon in the optical range, the reflectance at normal incidence is in the range of 0.3 to 0.4. Especially when the wavelength of the incoming light is in the ultra-violet range, the reflectance becomes high, and one should be careful of any stray light in the setup. This high reflectance can also influence the perceived spot size on the detector. The reflection of a small spot can be reflected back from the casing of the lens, and once arrived on the detector again, this reflection is a lot bigger than the original spot. 


\begin{comment}

To calculate the transmission and reflection on an interface between two mediums, imagine a parallel beam of light under an angle approaching an interface between two mediums. The angle of the incoming light in medium 1 is $\theta_i$, the angle of the light that is reflected is $\theta_r$, and the angle of the refracted light in medium 2 is $\theta_t$. The relation between the incoming light and the reflected light is given by the law of reflection: $\theta_i=\theta_r$, and the relation between the incoming and the refracted light is given by Snell's law: $n_1\sin(\theta_i)=n_2\sin(\theta_t)$. If one now also looks at the electric- and magnetic field within the two mediums, one can derive the fraction of reflected/transmitted intensity by solving the boundary conditions. The electric field is denoted as $E_j$, and the magnetic field is denoted as $H_j$ with $j\in{\left\{i,r,t\right\}}$ denoting respectively incoming, reflected, and transmitted. Two different cases can be considered, p- and s-polarisation. In the case of p-polarization, the electric field vector lies inside the plane of incidence, while in the case of s-polarisation the electric field vector is orthogonal to the plane of incidence. For p-polarisation, the boundary condition for the electric field is
\begin{equation}
    E_i\cos(\theta_i)+E_r\cos(\theta_i)=E_t\cos(\theta_t),
    \label{eq:Theory/EBoundary}
\end{equation}
and the boundary condition for the magnetic field is
\begin{equation}
    H_i-H_r=H_t.
    \label{eq:Theory/HBoundary}
\end{equation}
These two boundary conditions can only be solved by using the relation between the electric field and the magnetic field for a propagating wave describing photons. This relation is derived from the Maxwell equations and states $H=\sqrt{\epsilon/\mu}E$. The real part of the refractive index can be expressed as $n=c\sqrt{\epsilon \mu}$. Using these two expressions, the magnetic field can be expressed in terms of the electric field as
\begin{equation}
    H_{i,r}=\frac{n_1E_i}{\mu_1c} \ \ ; \ \ H_t=\frac{n_2E_t}{\mu_2 c}.
\end{equation}
Therefore \autoref{eq:Theory/HBoundary}, can be rewritten as
\begin{equation}
    \frac{n_1\left( E_i - E_r \right)}{\mu_1 c}=\frac{n_2E_t}{\mu_2 c}.
    \label{eq:Theory/MagneticFieldEq}
\end{equation}
Combining \autoref{eq:Theory/MagneticFieldEq} with \autoref{eq:Theory/EBoundary}, an expression for both the reflectance and the transmission can be found:
\begin{align}
    r_p&=\frac{\frac{n_1}{\mu_1}\cos(\theta_t)-\frac{n_2}{\mu_2}\cos(\theta_i)}{\frac{n_1}{\mu_1}\cos(\theta_t)+\frac{n_2}{\mu_2}\cos(\theta_i)}\approx \frac{n_1\cos(\theta_t) - n_2\cos(\theta_i)}{n_1\cos(\theta_t)+n_2\cos(\theta_i)}, \\ 
    t_p&=\frac{2\frac{n1}{\mu_1}\cos(\theta_i)}{\frac{n_1}{\mu_1}\cos(\theta_t)+\frac{n_2}{\mu_2}\cos(\theta_i)}\approx \frac{2n_1\cos(\theta_i)}{n1\cos(\theta_t)+n_2\cos(\theta_i)}.
\end{align}
In the optical range, most mediums are non-magnetic, and thus it can be assumed that $\mu_1=\mu_2=\mu_0$. Therefore, $\mu_0$ drops out of the equations for the reflectance and the transmission. 

For s-polarised light, the boundary conditions are slightly different. The boundary condition for the electric field now is
\begin{equation}
    E_i+E_r=E_t,
\end{equation}
and the boundary condition for the magnetic field is 
\begin{equation}
    -H_i\cos(\theta_i)+H_r\cos(\theta_i)=-H_t\cos(\theta_t).
\end{equation}
Now making the same steps as with the p-polarisation, the reflectance and transmission can be expressed as
\begin{align}
    r_p&= \frac{n_1\cos(\theta_i) - n_2\cos(\theta_t)}{n_1\cos(\theta_i)+n_2\cos(\theta_t)}, \\ 
    t_p&= \frac{2n_1\cos(\theta_i)}{n1\cos(\theta_i)+n_2\cos(\theta_t)}.
\end{align}
These equations are commonly known as the Fresnel equations. These expressions in their current form only are correct when the imaginary part of the refractive index $n'$ is zero. However, by taking the absolute values of the refractive index, they can also be applied to mediums where the imaginary part is non-zero. 

As is discussed earlier, the intensity does not scale linearly with the electric field amplitude. Therefore the intensity of the reflection is not simply given by $r$. The intensity reflection $R$ is given by
\begin{equation}
    R=\frac{\abs{E_r}^2}{\abs{E_i}^2}=\abs{r}^2.
\end{equation}
The intensity transmission is now given by the fraction that is not reflected: $T=1-R$.

Using these expressions for the reflectance, the reflectivity of silicon can be calculated. In the case of silicon in the optical range, the reflectance at normal incidence is in the range of 0.3 to 0.4. Especially when the wavelength of the incoming light is in the ultra-violet range, the reflectance becomes high, and one should be careful of any stray light in the setup. This high reflectance can also influence the perceived spot size on the detector. The reflection of a small spot can be reflected back from the casing of the lens, and once arrived on the detector again, this reflection is a lot bigger than the original spot. 
\end{comment}








